Deconfounding Duration Bias in Watch-time Prediction for Video Recommendation

Watch-time prediction remains to be a key factor in reinforcing user engagement via video recommendations. It has become increasingly important given the ever-growing popularity of online videos. However, prediction of watch time not only depends on the match between the user and the video but is often mislead by the duration of the video itself. With the goal of improving watch time, recommendation is always biased towards videos with long duration. Models trained on this imbalanced data face the risk of bias amplification, which misguides platforms to over-recommend videos with long duration but overlook the underlying user interests. This paper presents the first work to study duration bias in watch-time prediction for video recommendation. We employ a causal graph illuminating that duration is a confounding factor that concurrently affects video exposure and watch-time prediction -- the first effect on video causes the bias issue and should be eliminated, while the second effect on watch time originates from video intrinsic characteristics and should be preserved. To remove the undesired bias but leverage the natural effect, we propose a Duration Deconfounded Quantile-based (D2Q) watch-time prediction framework, which allows for scalability to perform on industry production systems. Through extensive offline evaluation and live experiments, we showcase the effectiveness of this duration-deconfounding framework by significantly outperforming the state-of-the-art baselines. We have fully launched our approach on Kuaishou App, which has substantially improved real-time video consumption due to more accurate watch-time predictions.

==> model_fig.tex <==
% transformer 局部放大？
\tikzset{
  mlp/.style = {draw=none, rectangle, fill=yellow3, minimum width=2cm, minimum height=1cm},
  embedding/.style = {draw=none, rectangle, fill=yellow2, minimum width=2cm, minimum height=0.5cm},
  input/.style = {draw=none, rectangle, fill=yellow1, minimum width=2cm, minimum height=1cm},
  input2/.style = {draw=none, rectangle, fill=blue1, minimum width=2cm, minimum height=1cm},
  output/.style = {draw=none, rectangle, fill=blue3, minimum width=1cm, minimum height=0.5cm},
  relu/.style = {draw=none, rectangle, fill=yellow3, minimum width=3.5cm, minimum height=0.15cm},
  concat/.style = {draw=none, rectangle, fill=yellow3, minimum width=15.0em, minimum height=0.15cm},
  relu2/.style = {draw=none, rectangle, fill=yellow2, minimum width=2.5cm, minimum height=0.15cm},
  sigmoid/.style = {draw=none, rectangle, fill=yellow1, minimum width=1.5cm, minimum height=0.15cm},
  temb6/.style = {draw=none, rectangle, fill=yellow4, minimum width=0.75cm, minimum height=0.25cm},
  embholder/.style = {draw=none, rectangle, minimum width=0.3cm, minimum height=0.3cm},
  smallembholder/.style = {draw=none, rectangle, minimum width=0.4cm, minimum height=0.4cm},
  mhtaholder/.style = {draw=none, rectangle, minimum width=0.4cm, minimum height=0.4cm},
  softmax/.style = {circle, draw, line width=0.5pt, minimum size=1.0em, inner sep=0pt, align=center},
  mhta/.style = {draw, rectangle, fill=yellow3, minimum width=15.0em, minimum height=0.2cm},
  topk/.style = {draw, rectangle, fill=yellow3, minimum width=15.0em, minimum height=0.2cm},
  mhta2/.style = {draw, rectangle, fill=yellow3, minimum width=10.0em, minimum height=0.2cm},
  bits/.style = {draw, rectangle, fill=blue1, minimum width=0.35cm, minimum height=0.35cm},
  bits2/.style = {draw, rectangle, fill=blue2, minimum width=0.35cm, minimum height=0.35cm},
  line/.style={->,shorten >=0.01cm,shorten <=0.01cm},thick,
  crossline/.style = {draw, -latex'},
  connector/.style = {draw,circle,node distance=3cm,fill=yellow!20}
}



\begin{figure*}[htb]
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[]

\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is  the standard layer)
% 全局的距离



% 基准点们
\node[] (firstnode) at (0,0) {};
\node[mlp, above of=firstnode, node distance=1.2cm] (mlp_1) {\LARGE $\text{MLP}_1$};
\node[mlp, right of=mlp_1, node distance=2.2cm] (mlp_2) {\LARGE $\text{MLP}_2$};
\node[right of=mlp_2, node distance=1.5cm] (dot) {\LARGE $\cdot\cdot\cdot$};
\node[mlp, right of=dot, node distance=1.5cm] (mlp_10) {\LARGE $\text{MLP}_{10}$};


\node[embedding,below of=mlp_10, node distance=1.5cm] (embedding_1) {\LARGE Embedding};
\node[input,below of=embedding_1, node distance=1.5cm,text width=1cm,align=center] (idinput) {\LARGE ID\\ Input};

\node (holder) at ($(mlp_1)!0.5!(mlp_2)$) {};
\node[input,text width=1cm,align=center] (denseinput) at (holder |- idinput) {\LARGE Dense\\ Input};

\node[output, above of=mlp_1, node distance=2.2cm] (output_1) {\LARGE $\text{Output}_1$};
\node[output, above of=mlp_2, node distance=2.2cm] (output_2) {\LARGE $\text{Output}_2$};
\node[above of=dot, node distance=2.2cm] (dot_2) {\LARGE $\cdot\cdot\cdot$};
\node[output, above of=mlp_10, node distance=2.2cm] (output_10) {\LARGE $\text{Output}_{10}$};


\node[above of=output_1, node distance=1.2cm] (label_1) {\LARGE $\widehat{\Phi}_k(1)$};
\node[above of=output_2, node distance=1.2cm] (label_2) {\LARGE $\widehat{\Phi}_k(2)$};
\node[above of=output_10, node distance=1.2cm] (label_10) {\LARGE $\widehat{\Phi}_k(10)$};

\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(denseinput.north)$) -- ($(mlp_1.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(denseinput.north)$) -- ($(mlp_2.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(denseinput.north)$) -- ($(mlp_10.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(idinput.north)$) -- ($(embedding_1.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(embedding_1.north)$) -- ($(mlp_10.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(embedding_1.north)$) -- ($(mlp_1.south)$);
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(embedding_1.north)$) -- ($(mlp_2.south)$) ;

\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(mlp_1.north)$) -- ($(output_1.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(mlp_2.north)$) -- ($(output_2.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(mlp_10.north)$) -- ($(output_10.south)$) ;

\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]},densely dotted] ($(label_1.south)$) -- ($(output_1.north)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]},densely dotted] ($(label_2.south)$) -- ($(output_2.north)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]},densely dotted] ($(label_10.south)$) -- ($(output_10.north)$) ;


% bbbbbbbbbbbbbbbbbbbb


\node[mlp, right of=mlp_10, node distance=7.0cm] (sharedmlp_1) {\LARGE Shared MLP};

\node[embedding, below of=sharedmlp_1, node distance=1.5cm] (embedding_b) {\LARGE Embedding};

\node[left of=embedding_b, node distance=1.5cm] (embedding_b_west) {};
% \node[right of=embedding_b, node distance=1.5cm] (embedding_b_east) {};

\node[input, below of=embedding_b_west, node distance=1.5cm, text width=1cm,align=center] (duration) {\LARGE ID\\ Input};
\node[input2, right of=duration, node distance=2.5cm] (idinput_b) {\LARGE Duration};
\node[input, left of=duration, node distance=2.5cm, text width=1cm,align=center] (denseinput_b) {\LARGE Dense\\ Input};

\node[output, above of=sharedmlp_1, node distance=2.2cm] (output_b) {\LARGE $\text{Output}$};


\node[above of=output_b, node distance=1.2cm] (label_b) {\LARGE $[\widehat{\Phi}_k(1),\widehat{\Phi}_k(2),\cdot\cdot\cdot, \widehat{\Phi}_k(10)]$};

\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(denseinput_b.north)$) -- ($(sharedmlp_1.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(duration.north)$) -- ($(embedding_b.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(idinput_b.north)$) -- ($(embedding_b.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(embedding_b.north)$) -- ($(sharedmlp_1.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(sharedmlp_1.north)$) -- ($(output_b.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]},densely dotted] ($(label_b.south)$) -- ($(output_b.north)$) ;



% ccccccccccccccccc

\node[mlp, right of=sharedmlp_1, node distance=7.0cm] (sharedmlp_2) {\LARGE Shared MLP};
\node[mlp, right of=sharedmlp_2, node distance=3.0cm] (residual_mlp) {\LARGE Residual MLP};

\node[embedding, below of=sharedmlp_2, node distance=1.5cm] (embedding_c1) {\LARGE Embedding};
\node[embedding, below of=residual_mlp, node distance=1.5cm] (embedding_c2) {\LARGE Embedding};

\node[input2, below of=embedding_c2, node distance=1.5cm] (duration_c) {\LARGE Duration};
\node[input, below of=embedding_c1, node distance=1.5cm, text width=1cm,align=center] (idinput_c) {\LARGE ID\\ Input};
\node[input, left of=idinput_c, node distance=2.5cm, text width=1cm,align=center] (denseinput_c) {\LARGE Dense\\ Input};

\node[] (output_c_holder) at ($(sharedmlp_2)!0.5!(residual_mlp)$) {};


\node[softmax, above of=output_c_holder, node distance=1.2cm] (add_c) {\Large +};


\node[output, above of=output_c_holder, node distance=2.2cm] (output_c) {\LARGE $\text{Output}$};


\node[above of=output_c, node distance=1.2cm] (label_c) {\LARGE $[\widehat{\Phi}_k(1),\widehat{\Phi}_k(2),\cdot\cdot\cdot, \widehat{\Phi}_k(10)]$};

\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(denseinput_c.north)$) -- ($(sharedmlp_2.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(idinput_c.north)$) -- ($(embedding_c1.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(duration_c.north)$) -- ($(embedding_c2.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(embedding_c2.north)$) -- ($(residual_mlp.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(embedding_c1.north)$) -- ($(sharedmlp_2.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(embedding_c2.north)$) -- ($(sharedmlp_2.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(sharedmlp_2.north)$) -- ($(add_c.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(residual_mlp.north)$) -- ($(add_c.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(add_c.north)$) -- ($(output_c.south)$) ;
\draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]},densely dotted] ($(label_c.south)$) -- ($(output_c.north)$) ;


% 文字们
\node[below of=idinput_c, node distance=1.5cm] (c_name) {\LARGE (c) ~Res-D2Q};
\node[below of=duration, node distance=1.5cm] (b_name) {\LARGE (b) ~D2Q};
\node[left of=b_name, node distance=7.5cm] (a_name) {\LARGE (a) ~Naive-D2Q};

% 虚线框
\draw[dashed] ($(label_1.south west)$) rectangle ($(label_c.north east)$) node[pos=.5] (label_all) {};
\node[left of=label_1, node distance=1.5cm] (label_all_name) {\LARGE Label:};


% mlp层的连线
% \draw[-{Latex[length=2.2mm, line width=0.75mm, width=2.0mm]}] ($(concat.north)$) -- ($(relu1.south)$) ;

\end{tikzpicture}
}
    \caption{Different model architectures for estimating watch-time per duration group, \textit{i.e.,} $\widehat{\Phi}_k(h(u,v))$. Figure (a)  fits individual models to estimate watch-time per duration group. Figure (b) fits a single model across all duration groups, with labels of watch-time quantiles calculated via watch-time empirical distribution in the corresponding duration group. Figure (c) further utilizes duration information in the network architecture and consequently improves watch-time estimation. }
    \label{fig:model1}
\end{figure*}



==> newfig.tex <==
% \documentclass[sigconf]{acmart}


% \usepackage{tikz}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{backgrounds}
\usetikzlibrary{positioning, fit, mindmap, trees, calc, tikzmark, shapes}
\usetikzlibrary{shapes.arrows, fadings, automata, tikzmark, decorations.pathreplacing, patterns}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{intersections}
% \usepackage{tkz-euclide}

\input{color}

% \begin{document}


\tikzset{
  FARROW/.style={arrows={-{Latex[length=1.25mm, width=1.mm]}}},
  DFARROW/.style={arrows={{Latex[length=1.25mm, width=1.mm]}-{Latex[length=1.25mm, width=1.mm]}}},
  origin/.style = {circle, fill=monte_carlo, minimum width=1.8em, align=center, inner sep=0, outer sep=0, font=\scriptsize},
  aug1/.style = {circle, fill=flamingo!72, minimum width=1.8em, align=center, inner sep=0, outer sep=0, font=\scriptsize},
  aug2/.style = {circle, fill=casablanca, minimum width=1.8em, align=center, inner sep=0, outer sep=0, font=\scriptsize},
  encoder/.style = {rectangle, fill=Madang!82, minimum width=11em, minimum height=3em, align=center, rounded corners=3},
  emb_layer/.style = {rectangle, fill=languid_lavender!72, minimum width=11em, minimum height=2em, align=center, rounded corners=3},
  project/.style = {rectangle, fill=hint_green, minimum width=7em, minimum height=2.4em, align=center, rounded corners=2},
  v_rep/.style={
       rectangle split,
       rectangle split part align=base,
       rectangle split horizontal=true,
       rectangle split draw splits=true,
       rectangle split parts=7,
       rectangle split part fill={red!30, blue!20, athens_gray!80, matisse, silver},
       %rounded corners,
       draw=gray, %very thick,
       very thin,
       minimum height=2em,
       minimum width=3em,
       %text width=3cm,
       inner sep=2.5pt,
       text centered,
%       font=\tiny,
       text=gray,
       rounded corners=1
       },
}

\begin{figure*}
\resizebox{0.9\linewidth}{!}{
    \begin{tikzpicture}
    
    %label=above:8cm, label=below:16cm, label=right:8cm, label=left:8cm
    % shape border rotate=180
        
    \node[] (o) at (0, 0) {};
    
    \node [above of=o, node distance=0.8cm, align=center] (v_dots) {$\cdots$};
    \node [origin, left of=v_dots, node distance=0.6cm] (v2) {$v_2$};
    \node [origin, left of=v2, node distance=0.75cm] (v1) {$v_1$};
    \node [origin, right of=v_dots, node distance=0.6cm, inner sep=0, outer sep=0] (v4) {$v_{\scaleto{t-1}{2.8pt}}$};
    \node [origin, right of=v4, node distance=0.75cm] (v5) {$v_t$};
    
%    \node [thick, dotted, draw=black, fit={(v1) (v5)}, inner sep=3] (input) {};
    \node [emb_layer, above of=v_dots, node distance=1cm] (o_emb) {embedding layer};
    \node [encoder, above of=o_emb, node distance=1.2cm] (o_enc) {encoder~ $f(\cdot)$};
     \node [dashed, draw=black, fit={([yshift=-0.5mm, xshift=-0.5mm] o_emb.south west) ([yshift=0.5mm, xshift=0.5mm] o_enc.north east)}, inner sep=3] (o_m) {};
     
      \node[v_rep, rectangle split part fill={monte_carlo!62}, above of=o_enc, node distance=1.3cm] (v_i) {
      \nodepart{four} $\,\cdots$
     };
    
    \draw [thick,draw=black!42, decorate,decoration={brace,amplitude=8pt,mirror}] ([xshift=-1mm, yshift=-1mm] v1.south west) -- ([xshift=1mm, yshift=-1mm] v5.south east) node[midway,yshift=-0.5cm] (o_a) {{\small Original behavior sequence} $s$};
    
    
    \node [circle, fill=celestial_blue!72, right of=v5, node distance=3cm, minimum width=1.8em, align=center, inner sep=0, outer sep=0, font=\scriptsize] (v_t) {$v_{\scaleto{t+1}{2.8pt}}$};
    
    \node [emb_layer, above of=v_t, node distance=1cm, minimum width=6em] (t_emb) {embedding layer};
    
     \node[v_rep, rectangle split part fill={celestial_blue!48}, above of=t_emb, node distance=2.5cm] (t_r) {
      \nodepart{four} $\,\cdots$
     };
     
     \node [right of=v_i, node distance=1.5cm] (v_s) {$\bm{s}$};
     \node [left of=t_r, node distance=1.6cm] (t_o) {$\bm{v}_{t+1}$};
    
    %%%%%%%%%% augmentation 2 %%%%%%%%%%
    \node [left of=v1, node distance=4cm] (b_dots) {$\cdots$};
     \node [aug2, left of=b_dots, node distance=0.6cm] (b2) {$\widetilde{v}_2$};
    \node [aug2, left of=b2, node distance=0.75cm] (b1) {$\widetilde{v}_1$};
    \node [aug2, right of=b_dots, node distance=0.6cm, inner sep=0, outer sep=0] (b4) {$\widetilde{v}_{\scaleto{t-1}{2.8pt}}$};
    \node [aug2, right of=b4, node distance=0.75cm] (b5) {$\widetilde{v}_t$};
    \draw [thick,draw=black!42, decorate,decoration={brace,amplitude=8pt,mirror}] ([xshift=-1mm, yshift=-1mm] b1.south west) -- ([xshift=1mm, yshift=-1mm] b5.south east) node[midway,yshift=-0.5cm] (b_a) {$s^{a_j}$};
    
%    \node [thick, dotted, draw=black, fit={(b1) (b5)}, inner sep=3] (aug2) {};
    \node [emb_layer, above of=b_dots, node distance=1cm] (b_emb) {embedding layer};
    \node [encoder, above of=b_emb, node distance=1.2cm] (b_enc) {encoder~ $f(\cdot)$};
    \node [dashed, draw=black, fit={([yshift=-0.5mm, xshift=-0.5mm] b_emb.south west) ([yshift=0.5mm, xshift=0.5mm] b_enc.north east)}, inner sep=3] (b_m) {};
    
    \node[v_rep, rectangle split part fill={casablanca!62}, above of=b_enc, node distance=1.3cm] (v_b) {
    \nodepart{four} $\,\cdots$
     };
      \node [left of=v_b, node distance=1.6cm] (v_ba) {$\bm{s}^{a_j}$};
    
    %%% aug 1
    \node [left of=b1, node distance=4cm] (a1_dots) {$\cdots$};
    \node [aug1, left of=a1_dots, node distance=0.6cm] (a2) {$\widehat{v}_2$};
    \node [aug1, left of=a2, node distance=0.75cm] (a1) {$\widehat{v}_1$};
    \node [aug1, right of=a1_dots, node distance=0.6cm] (a4) {$\widehat{v}_{\scaleto{t-1}{2.8pt}}$};
    \node [aug1, right of=a4, node distance=0.75cm] (a5) {$\widehat{v}_t$};
    \draw [thick,draw=black!42, decorate,decoration={brace,amplitude=8pt,mirror}] ([xshift=-1mm, yshift=-1mm] a1.south west) -- ([xshift=1mm, yshift=-1mm] a5.south east) node[midway,yshift=-0.5cm] (a_a) {$s^{a_i}$};

%    \node [thick, dotted, draw=black, fit={(a1) (a5)}, inner sep=3] (aug1) {};
    \node [emb_layer, above of=a1_dots, node distance=1cm] (a_emb) {embedding layer};
    \node [encoder, above of=a_emb, node distance=1.2cm] (a_enc) {encoder~ $f(\cdot)$};
    \node [dashed, draw=black, fit={([yshift=-0.5mm, xshift=-0.5mm]a_emb.south west) ([yshift=0.5mm, xshift=0.5mm] a_enc.north east)}, inner sep=3] (a_m) {};
    
    \node[v_rep, rectangle split part fill={flamingo!62}, above of=a_enc, node distance=1.3cm] (v_a) {
    \nodepart{four} $\,\cdots$
     };
     
     \node [right of=v_a, node distance=1.6cm] (v_aa) {$\bm{s}^{a_i}$};
     
    
     \draw[DFARROW, dashed] (a_m) -- (b_m) node [pos=0.5, above, black] (ab){share};
     \draw[DFARROW, dashed] (b_m) -- (o_m) node [pos=0.5, above, black] {share};
     
     
     %%%%% framework
     \node [above of=v_a, node distance=1cm, xshift=26.75mm] (cl_score) {$\bm{s}^{a_i} \cdot \bm{s}^{a_j}$};
     \node [above of=cl_score, node distance=0.8cm] (cl_loss) {contrastive loss};
     \draw[FARROW] (cl_score) -> (cl_loss);
     \draw[FARROW, rounded corners,] (v_a.north) |- (cl_score.west) {} ;
     \draw[FARROW, rounded corners,] (v_b.north) |- (cl_score.east) {} ;
     
     \node [above of=v_i, node distance=1cm, xshift=21.75mm] (rec_score) {$\bm{s} \cdot \bm{v}_{t+1}$};
     \node [above of=rec_score, node distance=0.8cm] (rec_loss) {recommendation loss};
     \draw[FARROW] (rec_score) -> (rec_loss);
     \draw[FARROW, rounded corners,] (v_i.north) |- (rec_score.west) {} ;
     \draw[FARROW, rounded corners,] (t_r.north) |- (rec_score.east) {} ;
    
     \foreach \x in {1,2,4,5}
     {
        \draw[FARROW] (a\x) -- ++(0, 0.7);
        \draw[FARROW] (b\x) -- ++(0, 0.7);
        \draw[FARROW] (v\x) -- ++(0, 0.7);
        \draw[FARROW] ($(a\x.north)+(0, 1.03)$) -- ++(0, 0.4);
        \draw[FARROW] ($(b\x.north)+(0, 1.03)$) -- ++(0, 0.4);
        \draw[FARROW] ($(v\x.north)+(0, 1.03)$) -- ++(0, 0.4);
     }
     \draw[FARROW] (v_t) -> (t_emb);

    \draw[FARROW] (a_enc) -> (v_a);
    \draw[FARROW] (b_enc) -> (v_b);
    \draw[FARROW] (o_enc) -> (v_i);
    \draw[FARROW] (t_emb) -> (t_r);
    \draw[FARROW, dashed] (o_a.south) -- ++(0, -0.3) -- ++(-5.3, 0) -> ++(0, 0.4);
    \draw[FARROW, dashed] (o_a.south) -- ++(0, -0.3) -- ++(-10.7, 0) -> ++(0, 0.4);
    
    \node [right of=a_a, node distance=1.7cm, yshift=-3mm] (aug_1) {$a_i \sim \mathcal{A}$};
    \node [right of=b_a, node distance=1.7cm, yshift=-3mm] (aug_1) {$a_j \sim \mathcal{A}$};
    
    
    \end{tikzpicture} }
    \caption{contrastive learning for rec}
    \label{fig:multitask}
\end{figure*}





% \end{document}
